The accuracy vs. coverage trade-off in patient-facing diagnosis models

A third of adults in America use the Internet to diagnose medical concerns, and online symptom checkers are increasingly part of this process. These tools are powered by diagnosis models similar to clinical decision support systems, with the primary difference being the coverage of symptoms and diagnoses. To be useful to patients and physicians, these models must have high accuracy while covering a meaningful space of symptoms and diagnoses. To the best of our knowledge, this paper is the first in studying the trade-off between the coverage of the model and its performance for diagnosis. To this end, we learn diagnosis models with different coverage from EHR data. We find a 1\% drop in top-3 accuracy for every 10 diseases added to the coverage. We also observe that complexity for these models does not affect performance, with linear models performing as well as neural networks.

==> old_sections/intro_tmp.tex <==

Consider the following scenario: X is experiencing frequent urination with burning sensation and has some belly pain and mild fever. Does X needs to see a doctor? Or What if X has access to no doctors nearby or have no financial ability to see one?  What are the possibilities for this patient? Can she can get an actionable quality outcome? This is a common scenario  among 30\% of working age adult population in the US who have no or little health insurance. According to WHO, nearly half of the world population do not have access to healthcare \footnote{https://www.who.int/news-room/detail/13-12-2017-world-bank-and-who-half-the-world-lacks-access-to-essential-health-services-100-million-still-pushed-into-extreme-poverty-because-of-health-expenses}.  

A viable solution to this has been the emergence of online symptom checkers; symptom checkers are patient-facing applications that operates on the central premise that when a patient is educated on their possible health conditions based on their symptoms, then it becomes easier to follow through on the next steps to get the care, if necessary. These systems takes as input the set of symptoms input by the patients, asks a series of questions that are relevant to their symptoms and answerable by them. Then, it provides differential diagnosis (ranked list of diseases) that helps educate patients on the possible health conditions. In the above example, these symptom checkers may result in a differential diagnosis consisting of  "urinary tract infection" and "Pyelonephritis".  In this case, the patient may need to go into the doctor's office to get their prescription.


Why is it interesting and important?
There has been a number of recent studies on symptom checkers \cite{Semigran, razzaki18}. In these works, the focus has been on measuring the accuracy of the symptom checkers and very little discussion on the methodologies underpinning them. %As an example, \cite{Semigran} evaluated 50 symptom checkers;  each of them were treated as a blackbox for the purpose of evaluation. % treating them as blackboxes, and applying custom user-facing representations of 45 labeled clinical vignettes. Each clinical vignette is a brief summary of the patient condition, and the label is the top likely disease for that condition. Since symptom checkers take as input user-facing symptoms, the cases were converted to a set of symptoms.

While these studies shed light on the effectiveness or lack of, of the symptom checkers, very little is discussed about the importance of the backbone of these symptom checkers - namely about the user-facing symptoms and diagnosis labels and the model that captures their relationships. %However, there has been little work in understanding the impact of available symptoms and disorders or the algorithm that is used to arrive at the label.

Since the choice of outputs is a key design choice, in this paper, we explore the trade-off space where the number of diagnosed disorders varies in total number and complexity, and measure how that impacts end model performance for diagnosis. This calls for a large collection of clinical vignettes from which we can learn models; one approach is to curate clinical vignettes which is a costly and often infeasible endeavor. The other approach, which we take in this paper, is to use electronic health records that provides access to patient clinical cases.

We are not aware of any prior work that explicitly studies the trade-offs in learning diagnosis models used in the context of building symptom checkers. Most existing diagnosis learned from Electronic health record focus on a complementary task of ICD code prediction that is often used in the context of billing. A disease is defined by a higher state that encompasses multiple codes and other electronic phentotypes (see \S~\ref{sec:phenotypes} on further discussion). Also, previous models have used the entirety of patient clinical notes or structured data both of which are unhelpful in the context of symptom checkers.


Here are the key contributions of our work:
\begin{itemize}
    \item Describe how electronic health records can be used to build symptom checkers
    \item Study the trade-off between number of disorders and accuracy of the model
    \item Study the trade-off between number of symptoms and accuracy of the model
\end{itemize}



%What are the key components of my approach and results? Also include any specific limitations.




%Access to best healthcare is a largely unsolved problem across the globe. In the US alone, there is staggering 30\% of working age adult population \TODO{Cite} with no or little health insurance to cover their visits to the doctors. In the developing and undeveloped parts of the world, the numbers are only staggering. 
%With increasing availability of internet across the globe, a viable alternative has been telehealth. There are already hospitals \TODO{cite rural areas with telehealth network} and early-stage startups aiming at scaling healthcare access to everyone.  \TODO{Expand here}



%Lets start with a scenario: A patient with access to no doctors nearby or have no financial ability to see one is experiencing a certain set of symptoms:frequent urination with burning sensation, and abdominal pain with mild fever. What are the possibilities for this patient? Can she can get an of actionable quality outcome in the confines of her room? A scenario such as this is common among 30\% of working age adult population who have no or little health insurance, and these statistics is only strikingly bleak, when we consider world population. Access to best healthcare has increasingly becoming a luxury\TODO{provide stats}





%where the patients may not need in-clinic work-up, but can engage deeply with doctors, and partially automated systems \TODO{Cite}. The central premise is that a majority of acute conditions are resolvable online \TODO{check correctness and cite}. A core requirement of these systems is to enable certain amount of automation through an initial automated differential diagnosis: , the goal of which is to the understand the symptoms that the user is experiencing, gather more information and identify a possible set of diagnosis (differential diagnosis). 

%We want to differentiate the "symptom-checkers" available online, including the many that were studied in the paper of \cite{semigran_comparison_2016}. For these symptom-checkers, diagnosis based on symptoms is the end-task. In contrast, in telehealth supported by many platforms such as Babylon, Ada, K-health, or FirstOpinion, symptom checkers is a starting point for user-doctor interaction. However, based on differential, the patients can choose to exit the system,  without following-through with a doctor. This means that accuracy of the differential diagnosis provided by these systems is still quite important. As discussed in \TODO{cite}, false negatives, especially when life-threatening, can be quite dangerous. Similarly, overlly cautious systems can also unnecessarily scare the patients to be more hypochondriac.

%Sadly, there is no publications that are available that discusses the challenges and the ingredients in building such a system. Not surprisingly, for understandable reasons of competitive advantage, the work of \cite{Babylon} also provides a bird's eye of the internals of their system.


%How can we define models for differenttial diagnosis? One approach is to manually create relationship between symptoms and diseases - an approach of the expert systems and that of recent work of \cite{Babylon}. Electronic health records provide a source of data where there are patient level information and the medical expert is making a diagnosis. The natural question is what it takes to build a differential diagnosis model from EHR.

%In this paper, we explore what it takes to learn a differential diagnosis model from electronic health records. \TODO{expand why we are diffetn}




%With rapid proliferation of internet, new generation of telehealth \TODO{cite} are emerging as a viable alternative. In this set-up, for most patients, a initial work-up for the patients are done online by an automated decision support system  The central premise of these systems is that for a number of acute conditions, a visit to doctor's office is unnecessary and a resolution of actionable steps including an treatment option can be discerned online \TODO{cite}. When done correctly, telehealth has the immense potential to change the landscape of healthcare access \

%To ensure the safety of medical mobile apps, the US Congress is considering the regulation of apps that “provide a list of possible medical conditions and advice on when to consult a health care provider.




%The data set used in evaluation of the study had been released and recently, Babylon reported performance of their algorithm, albeit raising some controversies. 


We are not aware of any prior work that explicitly studies the trade-offs in learning diagnosis models used in the context of building symptom checkers. Most existing diagnosis learned from Electronic health record focus on a complementary task of ICD code prediction that is often used in the context of billing. A disease is defined by a higher state that encompasses multiple codes and other electronic phentotypes (see \S~\ref{sec:phenotypes} on further discussion). Also, previous models have used the entirety of patient clinical notes or structured data both of which are unhelpful in the context of symptom checkers.

The availability of EHR has given us access to patient level clinical information including their symptoms and disease. However, the accuracy of EHR data is not certain and are not as simple or straightforward as those cases curated by experts.  Patients can present with complex medical histories, be taking multiple medications, or have social risk factors that contribute to a constellation of findings not specifically associated with a single diagnosis.  Physicians may not know the diagnosis and would need to use more generalized versions of diagnostic codes (i.e. pneumonia versus mycoplasma pneumonia), or if they are unable to reach a certain diagnosis, end up using symptom-based diagnostic codes (i.e. heartburn versus gastroesophageal reflux)





The recent study of \cite{Semigran,} has been instrumental in bringing to foray the unreliability of existing symptom checkers.  However, due to the blackbox


focus has been on measuring the accuracy of the symptom checkers. While these studies shed light on the effectiveness (or lack) of the symptom checkers, very little is discussed about the technologies underpinning them. In particular, about the user-facing symptoms, the choice of diagnosis labels and the model that captures their relationships. 



==> old_sections/old_text.tex <==


\section{Methods}
We formulate clinical differential diagnosis as a classification task. We assume access to a labeled data set of $N$ clinical cases, $S = \{(\mathbf{x}_1, y_1), ... , (\mathbf{x}_N, y_N)\}$ derived from electronic health records. Each $x_n$ is an observed clinical case with $x_n \subset \mathcal{F}$, where $\mathcal{F}$ = \{$f_1$, \cdots , $f_K$\} is a set of $K$ findings and $y_n \in \{1, ..., L\}$ is the corresponding diagnosis.

\subsection{Dataset construction for model training}
\label{sec:training_set}
Here, we describe general approaches for automatically creating data sets for model training for diagnosis; the data sets are constructed using both expert systems and electronic health records. We evaluate the trained models on independent data sets described in \S~\ref{sec:exp}.

\noindent\textbf{Training set from EHR}
We represent entire EHR in temporal order: data is organized by patient and by time. Each patient may have different types of records, including encounters (visits with the doctor), medications, labs etc. For the purpose of this work, we use only the encounters. For a patient $p$, let  $\mathcal{T}_p = [e_{1,p}, \cdots e_{t,p}]$ represent their timeline (chronological ordering) of all their $t,p$ encounters. \TODO{FIGURE} provides an overview of the timeline a single patient. 

An important consideration in constructing clinical cases specific for a disease is to design electronic phenotypes that can serve as markers for that disease. We direct astute readers to \cite{Banda18} for in-depth discussion on electronic phenotyping and various approaches available. For the purpose of this paper, assume that for a disease $d$, the set of phenotypes, $\textrm{phenotype}(d)$ is available. Then, we consider encounters for a patient with that phenotype. We assign all the encounters with the temporal window for that diagnosis, assuming that the last visit corresponds to resolution of the condition. We define resolution to be when there has been at least $\tau$ days with no follow-up.  We construct a set of findings (user-focused) for that patient corresponding to that diagnosis from the clinical note corresponding to the first visit of that temporal window. In particular, we use the chief complaints and the HPI section.  
Algo.~\ref{algo:ehr} provides an overview of the algorithm for generating clinical cases for one disease at a time.

\begin{algorithm}
\begin{algorithmic}[1]
\State {\bf Input}: A disease $d$, its phenotypes $\textrm{phenotype}(d)$ and EHR: \{$\mathcal{T}_p$\}, resolution time $\tau$
\State {\bf Output}: A set of clinical cases $\mathcal{D}_d =  \{(x_1, d), \cdots ,(x_T , d )\}$ corresponding to disease $d$. 
\State $\mathcal{D}_d \gets \emptyset$
\State $\mathcal{P}$ $\leftarrow$ IDENTIFY-PATIENTS(\{$\mathcal{T}_p$\}, $S_d$)
\Comment{Select patients that have diagnosis d.}
\For{$p \in \mathcal{P}$} 
\State $(t_{s,p}, t_{e,p})$ $\leftarrow$ RESOLVED-DISEASE-TIME-WINDOW(p, $\mathcal{T}_p$,  $\textrm{phenotype}(d)$, $\tau$)
\State $x$ $\leftarrow$ EXTRACT-FINDINGS($t_{s,p}$)
\State $\mathcal{D}_d \gets  \mathcal{D}_d \cup (x,d)$
 \caption{Algorithm for constructing clinical cases for a single disease. }
  \label{algo:ehr}
 \end{algorithmic}
\end{algorithm}

The method IDENTIFY-PATIENTS identifies all the patients in EHR who satisfy the following two criteria: (1) the patient $p$ has an encounter $e_{k,p}$ with at lease one property in $S_d$ satisfied and (2) $e_{k,p}$ is an out-patient visit. The second requirement ensures that we focus on patients with disease manifestations with variant of disease, $d$.

The method RESOLVED-DISEASE-TIME-WINDOW identifies the temporal window of encounters for the patient $p$ that satisfies $\textrm{phenotype}(d)$ and also the problem is resolved for $\tau$.


Referring back to \TODO{FIGURE}, we also show an example of a clinical case constructed for a patient.

\noindent\textbf{Training set from expert system}
\label{sec:case_simulator}
% algorithm
\input{sections/simulator.tex}

Similar to the work of \cite{ravuri18}, wee also used the expert system to generate clinical cases. Algo.~\ref{algo:generator} provides an overview of the algorithm used to generate clinical cases.

\TODO{TODO: may want to include about identifiability, when we incorporate it}


\section{Experiments}

\subsection{Electronic Phenotyping}


\footnotesize
\begin{table*}
\centering
\begin{tabular}{ l| l| l }
\toprule
Disorder &	ICD9&	ICD10 \\
\midrule
strep throat&	034.0, 462&	J02.00, J02.9, J03.01, J03.00\\ 
allergic rhinitis&	477.0 477.1, 477.2, 477.8, 477.9& J30.1, J30.2, J30.5, J30.8, J30.81, J30.89, J30.9 \\
acute bronchitis&	466.0, 466.19	&J20.2, J20.3, J20.4, J20.5, J20.6, J20.7, J20.8, J20.9 \\ 
bacterial conjunctivitis&	372.03&	H10.31, H10.32, H10.33, H10.021, H10.022, H10.023, H10.029, H10.30\\ 
viral conjunctivitis&	077.99, 077.8, 077.3&	B30.0, B30.1, B30.2, B30.8, B30.9\\ 
infectious mononucleosis&	075&	B27.0, B27.00, B27.01, B27.02, B27.09, B27.90\\ 
constipation&	564.00, 564.01, 564.09&	K59.0, K59.00, K59.01, K59.02, K59.09\\ 
GERD	&530.11, 530.81 & K21.0, K21.9\\ 
migraine&	346.0, 346.1, 346.2, 346.4, 346.9&	G43, G43.1, G43.4, G43.5, G43.9\\ 
tension headache&307.81, 339.10	&G44.20, G44.201, G44.209, G44.21, G44.211, G44.219\\ 
cluster headache&339.00, 339.01&	G44.00, G44.001, G44.009, G44.01, G44.011, G44.019\\ 
acute gastroenteritis&	008.61, 008.62, 008.69, 008.8, 009.0, 009.1, 009.2, 009.3&	A09, A08.0,  A08.1, A08.2, A08.3, A08.4, A08.8\\ 
UTI	&599.0	&N39.0, N30.0, N30.9\\ 
Candidal vulvovaginitis &	112.1&	B37.3\\ 
Influenza	&487.1, 488.81, 488.82, 488.89, 497.1&	J09, J09.X1, J09.X2, J09.X3, J09.X0
\bottomrule
\end{tabular}
\caption{ICD codes that are used in electronic phenotypes for identifying the diagnosis for a patient. If at an encounter, a patient has been assigned a code (e.g. K21.9)  and did not do any subsequent follow-up in the next 30 days, then that encounter is used as a positive example for the corresponding disease (in this example, it will be GERD.}
\bottomrule
\end{table*}
\normalsize




\subsection{Dataset}

\noindent\textbf{Training set:} We use the approaches described in \S~\ref{sec:training_set} to generate training sets for model training. We focus on  \TODO{$K$} diseases that are common in outpatient clinics.

\TODO{describe the dataset -- years considered, number of data points}


{\bf specific details for EHR:} We constrained phenotypes to be ICD-9 and ICD-10 codes and used $\tau=30$ days for disease resolution.    We use the inhouse medical entity-extractor to identify the patient-facing symptoms/findings from the clinical notes.  \TODO{TODO: describe entity extractor}

\TODO{TODO: validate: We also explored if account visits prior to the diagnosis of interest to gather chief complaints. For acute, out patient visits, we found those pre-visits to be rare and hence did not pursue this approach}

{\bf specific details for Expert systems:} 
\\
\noindent\textbf{Evaluation set:}
We used two sources of data for evaluation.  The first is the Semigran dataset \cite{Semigran}. This dataset consists of 45 standardized patient clinical vignettes. The vignettes also have simplified inputs that are amenable to online symptom checkers. We used these simplified inputs for evaluation. The data sets had three categories of triage urgency: emergent care required (for example, pulmonary embolism), non-emergent care reasonable (for example, otitis media), and self care reasonable (for example, viral upper respiratory tract infection).

As a second data set for evaluation, we constructed an in-house clinical cases constructed by medical doctors. Note that the doctors were unaware of the exact strategy we uaed for  For each of the $K$ diseases in our training set, the doctors provided $N$ distinct clinical vignettes (in the form of structured findings) resulting in a total of $K\times N$ cases. \TODO{TODO: details of this data set}

\subsection{Metrics} 
We  report recall@k (k $\in \{5,10\}$). 
\begin{equation}
\textrm{recall@k} = \frac{\sum_{t=1}^{T} \sum_{j=1}^{j=K}[\hat{y}^{(t)}[j] = y^{(t)}] }{T},
\end{equation}
This metric (also called \emph{sensitivity}) is valuable in deployment contexts that involve aiding doctors in diagnosis, as it ensures that the relevant disease condition is considered within a small range of false positives.  

We also report mean of per-class accuracy ($\textrm{mca)}$. For a data set consisting of $C$ classes, with  $T_c$ examples in each class,  mean accuracy is the average of per-class accuracy:
\begin{equation}
\textrm{mca} = \frac{1}{C}\sum_{c}\frac{\sum_{t=1}^{T_c} I[\hat{y}^{(t)}[0] = y^{(t)}]}{T_k},
\end{equation}
where, for $t^{th}$ example, $\hat{y}^{(t)}[j]$ is the $j^{th}$ top class predicted from a model and $ y^{(t)}$ is its corresponding ground truth label, where $I$ denotes the indicator function.

\subsection{Next Steps}
See \href{https://docs.google.com/spreadsheets/d/1w_AG0Ore1oN-mLpwxsd_d6SVkAoiBe-M1k5TabJn9Fk/edit#gid=0}{google sheet} for next steps

\subection{Results}


\subsection{Qualitative Examples}


==> old_sections/simulator.tex <==

\begin{algorithm*}
\begin{algorithmic}[1]
\State {\bf Input}:Medical knowledge base with FREQ(d,f) and importance IMP(f); minimum disease prevalence $\beta$, $T$: number of clinical cases,  $K$: number of prevalent findings to add; $N$: number of random findings to add. $M$: number of findings to drop.
\State {\bf Output}: $\{{\bf s}^{(t)}, y^{(t)}\}_{t=1}^{T}$ pairs such that $y \in \mathcal{D}$ with  prevalence $\ge \beta$ and ${\bf s} \subset \mathcal{F}$ is the set of (noisy) findings manifested in a patient with disease $y$.  \\

\State FREQ(d,f) and IMP(d) are re-scaled using the non-linear weighting scheme described in \S\ref{sec:vddx} and lies between [0,1]
\State  $\mathcal{D}^{*} \gets \{d \in \mathcal{D} : prevalence(d) \ge \beta\} $  % \subseteq \mathcal{D}$ such that prevalance($d$) $\ge \beta \forall d  \in \mathcal{D}^{*}$  
\For{t = 1 to T} 
  \State  $y^{(t)} \sim  Uniform(\mathcal{D}^{*}) $ \Comment{Ground truth disease label for this case}
  \State ${\bf s}^{(t)} \gets \emptyset$
  \Comment{\TODO{this needs to be a set, and we choose one from multinomial}}
  \For{$f \in \textrm{Demographics}(\mathcal{F})$} \Comment{Demographic variables}
  	\If{ $f \in F^(*)$ and $rand() >  FREQ(f,y^{(t)})$}
  	 	\State $ {\bf s}^{(t)} \gets {\bf s}^{(t)} \cup  \{f\}$
  	 	\State $F^{*} \gets \textrm{RemoveMutex}(F^{*}, {\bf s}^{(t)})$ \Comment{remove mutual exclusives}
  
     \EndIf
   \EndFor 
   \State $F^{*} \gets  \mathcal{F} \setminus ( \textrm{Demographics}(\mathcal{F})$
    \While{$F^{*} \neq  \emptyset $}
    	\State $F^{*} \gets \textrm{RemoveTaboo}(F^{*}, {\bf s}^{(t)})$ \Comment{taboo findings}
    	 \State $F^{*} \gets \textrm{RemoveMutex}(F^{*}, {\bf s}^{(t)})$ \Comment{mutex findings}
    	\State $f \gets \textrm{GetNext}(F^{*})$
        \If {$rand() >  FREQ(f,y^{(t)})$}
    		\State $ {\bf s}^{(t)}  \gets {\bf s}^{(t)} \cup \{f\} $
            \State $F^{*} \gets F^{*} \setminus \{f\}$
 		\EndIf 
  	\EndWhile
  	\Comment{Optional} \\
    \State $ {\bf s}^{(t)} \gets \textrm{DropFindings}(M, {\bf s}^{(t)}) $\Comment{\TODO{Write method}}
    \State $ {\bf s}^{(t)} \gets \textrm{AddPrevalentFindings}(IMP, K, {\bf s}^{(t)}) $ 
    \State $ {\bf s}^{(t)} \gets \textrm{AddRandomFindings}(M, {\bf s}^{(t)}) $\Comment{\TODO{Write method}}

\EndFor
  \caption{Medical Case Simulator}
  \label{algo:generator}
 \end{algorithmic}
\end{algorithm*}

==> sections/icdcodes.tex <==
\begin{table*}
\centering
\begin{tabular}{ l| l| l }
\toprule
Disorder &	ICD9&	ICD10 \\
\midrule
\footnotesize
strep throat&	034.0, 462&	J02.00, J02.9, J03.01, J03.00\\ 
allergic rhinitis&	477.0 477.1, 477.2, 477.8, 477.9& J30.1, J30.2, J30.5, J30.8, J30.81, J30.89, J30.9 \\
acute bronchitis&	466.0, 466.19	&J20.2, J20.3, J20.4, J20.5, J20.6, J20.7, J20.8, J20.9 \\ 
bacterial conjunctivitis&	372.03&	H10.31, H10.32, H10.33, H10.021, H10.022, H10.023, H10.029, H10.30\\ 
viral conjunctivitis&	077.99, 077.8, 077.3&	B30.0, B30.1, B30.2, B30.8, B30.9\\ 
infectious mononucleosis&	075&	B27.0, B27.00, B27.01, B27.02, B27.09, B27.90\\ 
constipation&	564.00, 564.01, 564.09&	K59.0, K59.00, K59.01, K59.02, K59.09\\ 
GERD	&530.11, 530.81 & K21.0, K21.9\\ 
migraine&	346.0, 346.1, 346.2, 346.4, 346.9&	G43, G43.1, G43.4, G43.5, G43.9\\ 
tension headache&307.81, 339.10	&G44.20*, G44.21*\\ 
cluster headache&339.00, 339.01&	G44.00*, G44.01*\\ 
UTI	&599.0	&N39.0, N30.0, N30.9\\ 
Candidal vulvovaginitis &	112.1&	B37.3\\ 
Influenza	&487.1, 488.81, 488.82, 488.89, 497.1&	J09, J09.X1, J09.X2, J09.X3, J09.X0
\bottomrule
\end{tabular}
\caption{ICD codes that are used in electronic phenotypes for identifying the diagnosis for a patient. If at an encounter, a patient has been assigned a code (e.g. K21.9)  and did not do any subsequent follow-up in the next 30 days, then that encounter is used as a positive example for the corresponding disease (in this example, it will be GERD.}
\bottomrule
\end{table*}
\normalsize

==> sections/intro_old.tex <==
 30\% of the working-age adult population in the US have inadequate health insurance coverage and more than 12\% are uninsured\cite{CWF17}. Saddled by high deductibles and premiums, the under-insured population often faces the difficult decision between an expensive trip to the physician's office versus self-management with over-the-counter remedies and watchful waiting. Heightening this decision is the fact that early intervention and preventative care often leads to a faster recovery at lower cost. For instance, gastroesophageal reflux disease (known colloquially as heart burn) can be effectively treated early, which prevents the formation of Barett's esophagus, a more serious pre-cancerous disorder. However, with almost half of underinsured adults reporting debt incurred from medical costs\cite{}, it comes as no surprise that these patients are delaying their care.
 
Telehealth is emerging as an option for increasing access to preventive care for the under- and non-insured. Specifically, online symptom checkers can provide patients with easy access to information for guiding their decision-making. Patients input their symptoms into the system, and then the system asks a series of questions that are relevant to these symptoms. As an output, the symptom checker provides a differential diagnosis (ranked list of diseases) that helps educate patients on possible relevant health conditions. Patients can then use this information to help decide on the best course of action for their specific situation. 

Symptom checkers and diagnostic engines are also a means to alleviating healthcare costs by collecting pertinent data for the physician.  The set of questions a physician asks a patient is based off of the patient's chief complaint, the set of symptoms that the patient identifies as their main concerns.  A symptom checker works in the same fashion, taking in the user's chief complaint as the main input and generating a progression of questions. The physician and the symptom checker often asks the same questions in order to reach a similar differential diagnosis, suggesting that collecting patient reported information could be an automated process and help physicians be more efficient in caring for their patients.


\pagebreak

To be useful to patients and physicians, symptom checkers must have high accuracy, while covering a large space of symptoms and diseases. Accuracy is of paramount importance as an incorrect list of potential diagnoses would be useless to the patient or worse yet, give them unnecessary cause for concern. Furthermore, the symptom checker must understand both the symptoms the patient is experiencing and the corresponding diagnosis. Capturing the clinical meaning of the symptoms as it relates to various diagnosis is challenging in several ways.  

First is in understanding what the user is trying to describe.  Entering in "chest pressure" is straightforward, but what if it is described as "an elephant sitting on my chest"?  Should the latter description be considered "chest pressure", "chest discomfort", "chest tightness", "difficulty breathing", all of which could lead to different diagnoses?  Another consideration is how to understand the nuances among closely neighboring symptoms and how those relationships affect the potential diagnoses.  Should "chest pressure" be considered as relatively similar "chest tightness"?  Related to this is understanding the user's implied answers; for instance, if the user denies "chest discomfort", does that mean the system should not ask about other uncomfortable chest symptoms, such as "chest pressure" or "chest tightness"?  Furthermore, the system needs to cover all manner of diseases if it is able to properly create a list of diagnosis.  For the previous user, imagine if the system did not have a disease such as “asthma” or "myocardial infarction". Without understanding the pros and cons of these challenges, the symptom checker can suggest incorrect diagnosis that is detrimental to the users as it is almost impossible that the user would know what diseases are supported or important to be considered (the reason why they are using symptom checker, in the first place).

In this paper, we focus on the first important consideration in building diagnosis models. In particular, we are interested in understanding the trade-off space where the number of diseases varies in total number and complexity, and measure how that impacts end model performance for diagnosis. For understanding this trade-off, we use the clinical vignettes from \cite{semigran} and use the metrics outlined in \TODO{cite}.  To the best of our knowledge, this paper is the first in studying this trade-off in the context of user-facing diagnosis.  

To study this trade-off, we need a large collection of clinical vignettes from which we can learn models for diagnosis; one approach is to curate clinical vignettes \TODO{cite: Babylon} which is a costly and unfeasible endeavor. The other approach, which we take in this paper, is to use electronic health records that provides access to patient clinical cases. We discuss the challenges and the approach we took in constructing reliable training set for model training \TODO{Section}.

To summarize, the main contributions of our work include:
\begin{itemize}
    \item Introduce and study the importance of trade-off between number of disorders and the complexity of diagnosis in user-facing setting
    \item Introduce a methodology for building patient-facing symptom checkers from Electronic health records (\S ~\ref{sec:model})
    \item Present an approach to build clinical vignettes from EHR that can be used (\S ~\ref{sec:ehr})
    \item  \TODO{ discuss results} ~\ref{sec:results}
\end{itemize}





==> sections/methods_old.tex <==


\comment{
We used one-hot encoding to represent $\mathcal{X}$ for some of our models. Specifically, we define an $N \times 2K$ matrix, $M$, where the first $K$ columns of this matrix represent symptoms known to be present and the second $K$ columns represent symptoms known to be absent. Such that
\begin{equation}
    m_{i,j} = \begin{cases} 
      1 & x_{i,j}=1 \\
      0 & x_{i,j}\in {-1,0}
   \end{cases}
\end{equation}
and 
\begin{equation}
    m_{i, (j+K)} = \begin{cases} 
      1 & x_{i,j}=-1 \\
      0 & x_{i,j} \in {0,1}
   \end{cases}
\end{equation}

We trained three different models: a multi-class logistic regression, a fully connected multi-layer perceptron (MLP) and a neural network which uses an embedding layer. The diagrams of two of the models are shown below


\begin{figure}[H]
\centering
\includegraphics[scale=0.6]{figs/combined_diagram.png}
\label{fig:training_data}
\caption{Diagrams of the embedding (A) and MLP (B) models.}
\end{figure}

The embedding model (shown in Fig 2A) embeds the symptoms of the patient and then averages the embeddings of the symptoms. The MLP conducts one-hot encoding of the symptoms as described above and then passes the resulting matrix into a fully connected neural network.
}

==> sections/scope.tex <==
This focus of this paper is to understand the trade-offs in using EHR data to create a diagnosis model for use in an online symptom checker or for medical decision support. One of the most important trade-offs is related to the coverage of the diagnosis model: a very focused diagnosis model that can only distinguish between disease A and B can be very accurate. However, its lack of coverage would greatly limit its utility and place the burden on the patient to have some medical understanding of the checker's limitations. Physicians are trained to diagnose a variety of common diseases while still being able to recognize rarer diseases or flag clinical presentations that require urgent evaluation. Diagnosis engines need to emulate a physician's broad diagnostic reasoning.

The first trade-off to consider is between diagnostic accuracy and the number of diseases covered by the the symptom checker. In a manually curated diagnosis engine, increasing coverage is a complex and unscalable process. We propose taking a machine learning approach using EHR records. However, machine learning models tend to show declining accuracy as the number of possible classifications increases.
Furthermore, optimizing accuracy is also difficult due to how EHR data is structured.  Diagnostic labels on EHR data are often based on ICD codes which are in turn, primarily used for billing.  Substituting billing codes for diagnosis as ground truths could be misleading since they do not always represent the diagnosis.  EHR data is also collected from a variety of patients who often have multiple diseases or comorbid conditions that confounds the relationships between the findings and the diagnoses.  

Second, we are interested in the effects of using colloquial patient language, rather than medical language. Allowing patients to enter free text for symptoms (e.g. stomach pain, belly pain) provides a better user experience and allows the model to capture additional context. However, this text may need to be mapped to standardized medical concepts (e.g. abdominal pain) for adequate diagnostic accuracy. 

% The focus of this paper is in understanding this trade-off. We are interested in performing systematic study in understanding the trade-off involved in using building machine learning models for differential diagnosis, that can serve as backbone of symptom checkers. In particular, how does the performance of the diagnosis vary with number of diseases modeled? How does understanding of the symptoms guide differential diagnosis?

%Consider the following scenario: X experiences some belly pain, has the urge to use  the bathroom frequently, and has a burning sensation.  Does X needs to see a doctor?  What if X has access to no doctors nearby or lacks the sufficient financial ability to see one?  What are the possibilities for this patient? Can she can get an actionable quality outcome?  In the above scenario, the patient, without needing to go to the doctor, should be able to get a correct differential of "urinary tract infection" and "Pyelonephritis", both of which require immediate access to doctor to get the antibiotics needed to recover from urinary tract infection.

% This scenario requires that the symptom checker understands the patient-language of "belly pain" (abdominal pain, in medical terms) and "urge to use bathroom frequently" (frequent urination, in medical terms) in order to serve the user. In addition, belly pain is related to many other diseases including appendicitis and gastroenteritis. In similar vein, 
% “frequent urination”  to Benign prostatic hyperplasia or type 2 diabetes or overactive bladder How does the differential diagnosis change as a function of  diseases encoded in a machine learning model? 



The aim of this paper contrasts with previous works \cite{semigran_comparison_2016, razzaki18} where the emphasis was on benchmarking symptom checkers based on standardized medical terminology. To the best of our knowledge, none of these papers discussed the structure of the underlying models or the trade-offs involved in designing these models. Symptom checkers were used as black box for evaluation. While the exception is \cite{razzaki18}, this paper also did not provide details of underlying architecture or the insights into the disease and findings landscape. Given that the graphical model was manually tuned based on manually curated clinical vignettes, and the benchmark datasets were not openly available, it leaves the readers with much to imagine.



%In this paper, we instead pose diagnosis as a classification task, where the parameters of the classifier are learned from clinical cases obtained from electronic health records. This provides a mechanism for updating the model with new diseases, or with diseases that have different manifestations or different contexts (geographies, demographies, seasons, etc.).



==> sections/scope_old.tex <==
 \TODO{Aim to weave in a scenario where home treatment is sufficient}
 
 \TODO{this section needs some real love}
 
This focus of this paper is to understand the trade-offs in using EHR data to create a symptom checker.  While these trade-offs can be minimized by narrowing the scope of diseases recognized by the symptom checker, that would greatly limit its utility and place the burden on the patient to have some medical understanding of the checker's limitations.  Physicians are trained to diagnose a variety of common diseases while still being able to recognize rarer diseases or flag clinical presentations that require urgent evaluation.  To best serve the user, the symptom checker needs to emulate the physician's broad diagnostic reasoning to be of use to a user.  Imagine an uninsured user who presents with headaches and neck pain but hopes to avoid seeing a doctor unless medically necessary.  These symptoms could be due to a benign diagnosis of "tension headache" and "neck strain" which self-resolve with supportive care at home, or could potentially be due to "meningitis" which is a medical emergency.  A symptom checker that is not trained on recognizing both disorders would render it useless for this user.

With the aim of recognizing a large set of varied diseases, the first trade-off to consider is between diagnostic accuracy and the number of diseases covered by the the symptom checker. Machine learning models tend to show declining accuracy as the number of possible classifications increases. However, both high accuracy and good coverage of diseases are necessary for a symptom-checker to be usable by patients.  Optimizing accuracy is also difficult due to how EHR data is structured.  Diagnostic labels on EHR data are often based on ICD codes which are in turn, primarily used for billing.  Substituting billing codes for diagnosis as ground truths could be misleading since they do not always represent the diagnosis.  EHR data is also collected from a variety of patients who often have multiple diseases or comorbid conditions that confounds the relationships between the findings and the diagnoses.  

Second, we are interested in the effects of using colloquial patient language, rather than medical language. A priori, allowing patients to enter free text for symptoms (e.g. stomach pain, belly pain) provides a better user experience and allows the model to capture additional context. However, this text may need to be mapped to standardized medical concepts (e.g. abdominal pain) for adequate diagnostic accuracy. This mapping requires expensive manual curation; so ideally, the raw input from patients can be used rather than the normalized concepts. 

% The focus of this paper is in understanding this trade-off. We are interested in performing systematic study in understanding the trade-off involved in using building machine learning models for differential diagnosis, that can serve as backbone of symptom checkers. In particular, how does the performance of the diagnosis vary with number of diseases modeled? How does understanding of the symptoms guide differential diagnosis?

%Consider the following scenario: X experiences some belly pain, has the urge to use  the bathroom frequently, and has a burning sensation.  Does X needs to see a doctor?  What if X has access to no doctors nearby or lacks the sufficient financial ability to see one?  What are the possibilities for this patient? Can she can get an actionable quality outcome?  In the above scenario, the patient, without needing to go to the doctor, should be able to get a correct differential of "urinary tract infection" and "Pyelonephritis", both of which require immediate access to doctor to get the antibiotics needed to recover from urinary tract infection.

% This scenario requires that the symptom checker understands the patient-language of "belly pain" (abdominal pain, in medical terms) and "urge to use bathroom frequently" (frequent urination, in medical terms) in order to serve the user. In addition, belly pain is related to many other diseases including appendicitis and gastroenteritis. In similar vein, 
% “frequent urination”  to Benign prostatic hyperplasia or type 2 diabetes or overactive bladder How does the differential diagnosis change as a function of  diseases encoded in a machine learning model? 



The aim of this paper contrasts with previous works \cite{semigran_comparison_2016, razzaki18} where the emphasis was on benchmarking symptom checkers based on standardized medical terminology. To the best of our knowledge, none of these papers discussed the structure of the underlying models or the trade-offs involved in designing these models. Symptom checkers were used as black box for evaluation. While the exception is \cite{razzaki18}, this paper also did not provide details of underlying architecture or the insights into the disease and findings landscape. Given that the graphical model was manually tuned based on manually curated clinical vignettes, and the benchmark datasets were openly available, it leaves the readers with much to imagine.



%In this paper, we instead pose diagnosis as a classification task, where the parameters of the classifier are learned from clinical cases obtained from electronic health records. This provides a mechanism for updating the model with new diseases, or with diseases that have different manifestations or different contexts (geographies, demographies, seasons, etc.).


